DiaLoc: An Iterative Approach to Embodied Dialog Localization

Multimodal learning has advanced the performance for many vision-language tasks. However, most existing works in embodied dialog research focus on navigation and leave the localization task understudied. The few existing dialog-based localization approaches assume the availability of entire dialog prior to localizaiton, which is impractical for deployed dialog-based localization. In this paper, we propose DiaLoc, a new dialog-based localization framework which aligns with a real human operator behavior. Specifically, we produce an iterative refinement of location predictions which can visualize current pose believes after each dialog turn. DiaLoc effectively utilizes the multimodal data for multi-shot localization, where a fusion encoder fuses vision and dialog information iteratively. We achieve state-of-the-art results on embodied dialog-based localization task, in single-shot (+7.08% in Acc5@valUnseen) and multi-shot settings (+10.85% in Acc5@valUnseen). DiaLoc narrows the gap between simulation and real-world applications, opening doors for future research on collaborative localization and navigation.

==> section/todo.tex <==
\section{TODO list}
{\color{red}
\begin{itemize}
    \item novelty: 
    \begin{itemize}
        \item chaining dialogs
        \item uniform prediction without dialog
        \item language node contrastive learning, predict similarity. 
    \end{itemize}
    \item correctness:
    \begin{itemize}
        \item results on Test set: target floor and all floors
        \begin{itemize}
            \item linunet: target floor
            \item linuent: all floor
            \item our: target floor
            \item our: all floor
            \item our-turn: all floor
            \item our-turn: tar floor
        \end{itemize}
        \item upgrading baseline to use Bert encoder
    \end{itemize}
 \end{itemize }
 }
